Integer Programming as a General Solution Methodology for Path-Based Optimization in Robotics: Principles, Best Practices, and Applications

Integer programming (IP) has proven to be highly effective in solving many path-based optimization problems in robotics. However, the applications of IP are generally done in an ad-hoc, problem specific manner. In this work, after examined a wide range of path-based optimization problems, we describe an IP solution methodology for these problems that is both easy to apply (in two simple steps) and high-performance in terms of the computation time and the achieved optimality. We demonstrate the generality of our approach through the application to three challenging path-based optimization problems: multi-robot path planning (MPP), minimum constraint removal (MCR), and reward collection problems RCPs). Associated experiments show that the approach can efficiently produce (near-)optimal solutions for problems with large state spaces, complex constraints, and complicated objective functions. In conjunction with the proposition of the IP methodology, we introduce two new and practical robotics problems: multi-robot minimum constraint removal (MMCR) and multi-robot path planning (MPP) with partial solutions, which can be quickly and effectively solved using our proposed IP solution pipeline.

==> 2-related.tex <==
\section{Related Work}\label{sec:related}

Integer programming (IP) methods are already widely used to solve combinatorial optimization 
problems since decades ago~\cite{nemhauser1988integer}. The application of IP methods covers 
a variety section of problems, e.g., traveling salesperson problem~\cite{miller1960integer}, 
network flow~\cite{hu1969integer}, and multi-target tracking~\cite{morefield1977application}. 
More recent study provides applications of IP methods on path optimization 
problems in robotics area, e.g., multi-robot path planning 
\cite{schouwenaars2001mixed, peng2005coordinating, YuLav16TRO}, task and motion planning 
for robotics manipulators~\cite{ding2011mixed, han2017complexity}. 

\mpp finds applications in a diverse array of areas including assembly~\cite{HalLatWil00}, 
evacuation~\cite{RodAma10}, formation~\cite{PodSuk04,SmiEgeHow08}, 
localization~\cite{FoxBurKruThr00}, microdroplet manipulation
\cite{GriAke05}, object transportation~\cite{RusDonJen95}, search and 
rescue~\cite{JenWheEva97}, and human robot interaction~\cite{knepper2012pedestrian}, 
to list a few. In the past decade, significant progress has been made on {\em optimally} 
solving \mpp problems in discrete (graph-base) environments. 
Algorithm solutions for such a discrete \mpp are often through reduction to other problems 
\cite{Sur12,erdem2013general,YuLav16TRO}. 
Decoupling-based heuristics are also proven to be 
useful~\cite{StaKor11,wagner2015subdimensional,boyarski2015icbs}. 
Similar to the partial solution studied in this paper, a recent work~\cite{MaIJCAI18} provides 
a search-based solver which optimizes the number of robot that reach goals in a limited time horizon.

\mcr finds applications in constraint-based task and motion planning~\cite{lozano2014constraint, dantam2018incremental}, 
object rearrangement\cite{krontiris2016efficiently,han2017complexity},  and development of control strategies~\cite{castro2013incremental}. 
An initial study~\cite{hauser2014minimum} proves that \mcr is NP-hard, and provides two search-based solvers. 
The solvers in~\cite{hauser2014minimum} can be extended to handle the case in which the 
obstacles are weighted~\cite{garrett2015ffrob}. 
An approximate method in~\cite{krontiris2015computational} provides a desirable trade-off 
between minimizing constraints, path length and computational time. 
Recent studies on \mcr reduces the gap between computational lower and upper bound on 
producing optimal solutions~\cite{eiben2018improved}. 

\qcop, as it is introduced in~\cite{yu2016correlated}, is a nonlinear extension to the 
{\em orienteering problem}~\cite{vansteenwegen2011orienteering} in which the robot is tasked 
to collect spatially scattered rewards by physically visit their locations. In \qcop, the 
robot is able to collect partial rewards from locations near its path even if it does not 
visit these locations. \qcop is solved optimally by a {\em mixed integer quadratic planning} 
model introduced in~\cite{yu2016correlated}. In \otp~\cite{yu2014optimal}, a tourist (robot) is interested in 
visiting some {\em point of interests} (POIs) that are 
spatially distributed. The reward the robot collects at each POI is calculated by a function 
whose input is the time the robot stays at the POI. 
\qcop and \otp have close correlation to information gathering tasks. For example, 
precision agriculture~\cite{tokekar2016sensor}, monitoring environmental attributes of the 
ocean~\cite{ma2016information}, tourist route planning~\cite{gavalas2015heuristics}, 
and infrastructure inspection~\cite{papachristos2016distributed}. 
